Vermilion: A Traffic-Aware Reconfigurable Optical Interconnect with Formal Throughput Guarantees

The increasing gap between datacenter traffic volume and the capacity of electrical switches has driven the development of reconfigurable network designs utilizing optical circuit switching. Recent advancements, particularly those featuring periodic fixed-duration reconfigurations, have achieved practical end-to-end delays of just a few microseconds. However, current designs rely on multi-hop routing to enhance utilization, which can lead to a significant reduction in worst-case throughput and added overhead from congestion control and routing complexity. These factors pose significant operational challenges for the large-scale deployment of these technologies. We present Vermilion, a reconfigurable optical interconnect that breaks the throughput barrier of existing periodic reconfigurable networks, without the need for multi-hop routing -- thus eliminating congestion control and simplifying routing to direct communication. Vermilion adopts a traffic-aware approach while retaining the simplicity of periodic fixed-duration reconfigurations, similar to RotorNet. We formally establish throughput bounds for Vermilion, demonstrating that it achieves at least $33\%$ more throughput in the worst-case compared to existing designs. The key innovation of Vermilion is its short traffic-aware periodic schedule, derived using a matrix rounding technique. This schedule is then combined with a traffic-oblivious periodic schedule to efficiently manage any residual traffic. Our evaluation results support our theoretical findings, revealing significant performance gains for datacenter workloads.

==> macros.tex <==
%!TEX ROOT = main.tex
\usepackage{enumitem}

\makeatletter
 \renewcommand\subsubsection{\@startsection {subsubsection}{3}{\z@}%
     {-2.5ex \@plus -1ex \@minus -.2ex}%
     {1.3ex \@plus.2ex}%
    {\ACM@NRadjust\@subsubsecfont}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%     {-.75\baselineskip \@plus -.2\p@ \@minus -.2\p@}% before \@plus -2\p@ <<<
%     {.25\baselineskip}%
%     {\ACM@NRadjust\@secfont}}
% \@startsection {NAME}{LEVEL}{INDENT}{BEFORESKIP}{AFTERSKIP}{STYLE} 
%            optional * [ALTHEADING]{HEADING}
%    Generic command to start a section.  
%    NAME       : e.g., 'subsection'
%    LEVEL      : a number, denoting depth of section -- e.g., chapter=1,
%                 section = 2, etc.  A section number will be printed if
%                 and only if LEVEL gt or eq the value of the secnumdepth
%                 counter.
%    INDENT     : Indentation of heading from left margin
%    BEFORESKIP : Absolute value = skip to leave above the heading.  
%                 If negative, then paragraph indent of text following 
%                 heading is suppressed.
%    AFTERSKIP  : if positive, then skip to leave below heading,
%                       else - skip to leave to right of run-in heading.
%    STYLE      : commands to set style
%  If '*' missing, then increments the counter.  If it is present, then
%  there should be no [ALTHEADING] argument.  A sectioning command
%  is normally defined to \@startsection + its first six arguments.
\makeatother

% Colors
\definecolor{darkgreen}{rgb}{0.01, 0.75, 0.24}
\definecolor{darkcyan}{rgb}{0.0, 0.55, 0.55}
\definecolor{mycolor}{rgb}{0.01, 0.75, 0.24}

\definecolor{mygray}{gray}{0.9}
\definecolor{myred}{rgb}{0.75, 0, 0}

\definecolor{myblue}{HTML}{3ba9d1}
\definecolor{myyellow}{HTML}{d1c23b}
\definecolor{mydarkred}{HTML}{c27676}
\definecolor{mygreen}{HTML}{7dc276}

\definecolor{alg1}{rgb}{0.855, 1, 0.824}
\definecolor{alg2}{rgb}{1, 0.996, 0.824}
\definecolor{alg3}{rgb}{0.824, 0.914, 1}

% Comments 
\newcommand{\todo}[1]{\textcolor{darkcyan}{[TODO: #1]}}
\newcommand{\vk}[1]{\textcolor{red}{[VA: #1]}}
\newcommand{\stef}[1]{{\color{blue} {(SS: #1)}}}
\newcommand{\chen}[1]{{\color{darkgreen}{(CA: #1)}}}

% hypen
\mathchardef\hyphen="2D

% Formal
\newtheoremstyle{sltheorem}
{}                % Space above
{}                % Space below
{\slshape}        % Theorem body font % (default is "\upshape")
{}                % Indent amount
{\bfseries}       % Theorem head font % (default is \mdseries)
{.}               % Punctuation after theorem head % default: no punctuation
{ }               % Space after theorem head
{}                % Theorem head spec
\theoremstyle{sltheorem}
% \theoremstyle{plain}
\newtheorem{prop}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}
\newtheorem{observation}{Observation}
\newtheorem{condition}{Condition}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{Lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{property}{Property}
\newtheorem{paradox}{Paradox}
\newtheorem{heuristic}{Heuristic}
\newtheorem{conjecture}{Conjecture}

% For custom bold heading
\newcommand{\myitem}[1]{\vspace{1mm}\noindent\textbf{#1}}
\newcommand{\myitemit}[1]{\noindent\textit{#1}}
% \makeatletter\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}{3.25ex \@plus1ex \@minus.2ex}{-1em}{\normalfont\normalsize\itshape}}\makeatother

\newcommand{\remove}[1]{}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

% Some shortcuts for text
\newcommand{\first}{\emph{(i)}\xspace}
\newcommand{\second}{\emph{(ii)}\xspace}
\newcommand{\third}{\emph{(iii)}\xspace}
\newcommand{\fourth}{\emph{(iv)}\xspace}
\newcommand{\fifth}{\emph{(v)}\xspace}
\newcommand{\sixth}{\emph{(vi)}\xspace}
\newcommand{\seventh}{\emph{(vii)}\xspace}
\usepackage{xcolor}
\definecolor{light-gray}{gray}{0.9}
\usepackage{tcolorbox}
% \usepackage{soul}
% \newcommand{\mathcolorbox}[2]{\colorbox{#1}{$\displaystyle #2$}}


\newcommand{\First}{\emph{(I)}\xspace}
\newcommand{\Second}{\emph{(II)}\xspace}
\newcommand{\Third}{\emph{(III)}\xspace}
\newcommand{\Fourth}{\emph{(IV)}\xspace}
\newcommand{\Fifth}{\emph{(V)}\xspace}
\newcommand{\Sixth}{\emph{(VI)}\xspace}
\newcommand{\Seventh}{\emph{(VII)}\xspace}

\newcommand{\ie}{i.e., \@}
\newcommand{\eg}{e.g., \@}
\newcommand{\etc}{etc., \@}
\newcommand{\etal}{et al.\xspace}

\newcommand{\xref}[1]{\S\ref{#1}}
\newcommand{\axref}[1]{Appendix~\ref{#1}}
\newcommand{\cref}[1]{Chapter~\ref{#1}}
\newcommand{\pxref}[1]{(\xref{#1})}
\newcommand{\fref}[1]{Fig.~\ref{#1}}
\newcommand{\tref}[1]{Table~\ref{#1}}


% Notations
\makeatletter
\newcommand{\oset}[2]{%
  \mathop{#2}\limits^{
  \vbox to-.5\ex@{\kern-2\ex@
   \hbox{$\scriptstyle#1$}\vss}}}
\makeatother

% \makeatletter
% \newcommand{\oset}[3][-0.3ex]{%
%   \mathrel{\mathop{#3}\limits^{
%     \vbox to#1{\kern-2\ex@
%     \hbox{$\scriptstyle#2$}\vss}}}}
% \makeatother

% Notations
\newcommand{\degree}{\ensuremath{\hat{d}}\xspace}

% mathcal fonts
\def\M{\mathcal{M}}
\def\T{\mathcal{T}}

% Symbols
\newcommand*{\affaddr}[1]{\small{#1}}
\newcommand*{\affmark}[1][*]{\textsuperscript{#1}}
% \newcommand*{\email}[1]{\texttt{#1}}

\DeclareSymbolFont{extraup}{U}{zavm}{m}{n}
\DeclareMathSymbol{\varheart}{\mathalpha}{extraup}{86}
\DeclareMathSymbol{\vardiamond}{\mathalpha}{extraup}{87}
